Novel Representation Learning Technique using Graphs for Performance Analytics

The performance analytics domain in High Performance Computing (HPC) uses tabular data to solve regression problems, such as predicting the execution time. Existing Machine Learning (ML) techniques leverage the correlations among features given tabular datasets, not leveraging the relationships between samples directly. Moreover, since high-quality embeddings from raw features improve the fidelity of the downstream predictive models, existing methods rely on extensive feature engineering and pre-processing steps, costing time and manual effort. To fill these two gaps, we propose a novel idea of transforming tabular performance data into graphs to leverage the advancement of Graph Neural Network-based (GNN) techniques in capturing complex relationships between features and samples. In contrast to other ML application domains, such as social networks, the graph is not given; instead, we need to build it. To address this gap, we propose graph-building methods where nodes represent samples, and the edges are automatically inferred iteratively based on the similarity between the features in the samples. We evaluate the effectiveness of the generated embeddings from GNNs based on how well they make even a simple feed-forward neural network perform for regression tasks compared to other state-of-the-art representation learning techniques. Our evaluation demonstrates that even with up to 25% random missing values for each dataset, our method outperforms commonly used graph and Deep Neural Network (DNN)-based approaches and achieves up to 61.67% & 78.56% improvement in MSE loss over the DNN baseline respectively for HPC dataset and Machine Learning Datasets.

==> Background.tex <==
% Representation learning, feed-forward model. \\
% Most publicly available data sets that researchers use on machine learning models are in a tabular format due to the user-friendly interferences that make it easier to collect data from various applications. The machine learning researchers used many feature extraction models to understand the data better and achieve the predictive task required.  Approaches like using deep neural networks have been commonly used for the past couple of years. It showed a considerable improvement in predicting specific tasks way better than neural networks. Since then, it has been the main focus. Existing Tabular approaches need lots of labeled data, cannot self-regulate based on unlabeled samples, needs retraining when slightly different data samples get introduced to the model and considers each sample or a batch as input without leveraging the similarities or dissimilarities between the input samples regarding the predictive task.


% Recent research has found that neural network-based learning on graphs accommodates unlabeled data and outperforms traditional convolutional neural networks. The graph can learn to represent graph nodes, edges, and sub-graphs in low-dimensional vectors, which captures relationships across samples and parameters to embed the whole dataset effectively and learn from unlabeled samples by exploiting their similarities with other samples. The graph can be used in multiple tasks like Node Classification, Link Prediction, Community Detection, or Graph Classification.

% To generate a graph from a tabular dataset. We hypothesize that each node represents a sample with a unified embedding from individual sources. Leveraging neighborhood similarity measures to infer edges can yield cluster execution configurations that result in a similar performance. GNNs capture relationships across samples and parameters to create an effective embedding of the whole dataset and can learn from unlabeled samples by exploiting their similarities to others

==> ablation_study.tex <==
% \textbf{\textcolor{red}{Minimum Number of neighbours, $N$}}

% In the SGC and BGC approach, we have introduced a user-defined property minimum number of neighbors, which defines the minimum number of N neighbors of a node in the graph. This property maintains the graph connectivity and removes the potential risk of generating a disconnected graph. A sample's closest distance when computing cosine distance is the sample itself. Thus we have self-loops for all of the nodes in that graph. So, we choose the top $N + 1$ neighbors instead of the $N$. We then remove those self-loops from the induced graph as mentioned both in \ref{alg:scg} \& \ref{alg:bgc} \textbf{\textcolor{red}{PROPER MENTIONING OF REFERENCE NEEDED}}

% % Our study finds that, despite efficient memory improvements in \textbf{BGC} than that of \textbf{SCG}, \textbf{BGC} isn't suitable for very small-sized datasets. Conducting the BGC approach on a small-sized dataset may end in single-node graphs in generated clusters. We aim to preserve at least $N$ neighbors for each node of the induced graphs where N is always greater than 2. Thus, a single-node graph fails to achieve the integrity of our theory. Our study shows that at least 600 samples in a dataset are safe enough to conduct BGC. 

==> experimental_setup.tex <==

\subsection{System}
We run our experiments in parallel using two systems:
Penguin Computing On Demand (POD) and Google Colab.

\noindent
\textbf{Penguin Computing On Demand}
We use a system with 96 AMD EPYC CPUs. Each CPU has 8GB of RAM based on the 64-bit x86 architecture. The system also has 8-MI50 AMD GPUs with 512GB memory.

\noindent
\textbf{Google Colab}
We use a machine with Intel(R) Xeon(R) CPU with 26.75GB RAM and one NVIDIA Tesla P100 GPU with 16GB memory on Google Colab. Each CPU has 2.30GHz Intel (R) processing capability with two cores based on the x86 64 architecture. The GPUs are equipped with CUDA 11.2 toolkit. % by NVIDIA. 
\subsection{Dataset Description}
To thoroughly evaluate the benefit of our proposed graph construction and representation learning technique in HPC performance prediction tasks, we use three regression datasets collected on three different HPC facilities. Table~\ref{tab:datasets} presents a summary of all three datasets, the number of features and samples, the prediction target, and the type of ML task (regression). \textbf{Since typical HPC performance analytics tasks require predicting continuous values such as runtime, we focus solely on regression tasks in this work.}  
%Specifically, three datasets were collected from supercomputers in our previous research teamwork.

\noindent
\textbf{Catalyst: }
This dataset is %introduced in SC’19~\cite{patki2019performance}, and was the first such dataset to be 
collected from multiple systems using various user-level parameters on a production HPC cluster. %The features contain numerical values such as thread count and categorical values such as the algorithm used. 
The dataset contains %has various information since changes 
numerical information such as the number of nodes, cores per node, and service levels used during data collection across five benchmarks applications. This dataset will be published after the paper is accepted.

\noindent
\textbf{Vulcan: }
This publicly available dataset~\cite{tanzima_2019_3403038} captures all possible hardware performance counters of an open-source nuclear reactor simulation application, OpenMC~\cite{romano2013openmc}, by varying its input on an Intel Xeon Haswell system from a supercomputer in a production environment. The label of the dataset is the application's runtime. The features contain numerical values, including the number of threads running, number of cache misses, number of stall counters, and input size. %, and categorical values such as the application used. The dataset has various information since adjustments in the input size are introduced during the data collection process.

\noindent
\textbf{Cab: }
This publicly available dataset~\cite{tanzima_2019_3403038} is collected from a supercomputer in a production environment, capturing rich features that decide the process’s runtime. The features contain numerical values, including the number of faults, cache references and input size, and categorical values such as the application used. %The dataset has various information since changes in the input size were introduced during the data collection process. This dataset will be published after the paper is accepted.
\begin{table}[t]
\footnotesize
\caption{Dataset descriptions.}
\label{table:Datasets description}
\renewcommand{\arraystretch}{1.2}
\centering
\begin{tabular}{|p{1.3cm}|p{0.8cm}|p{0.85cm}|p{1cm}|p{0.9cm}|p{1.2cm}|}
\hline
Dataset	&Samples	&Features	&Domain	&Target	&Evaluation\\ \hline
Catalyst	&3992	&10	&HPC	&Runtime	&Regression (MSE)\\ \hline
Cab	&320	&148	&HPC	&Runtime	&Regression (MSE)\\ \hline
Vulcan	&321	&172	&HPC	&Runtime	&Regression (MSE)\\ \hline
\end{tabular}
\vspace{-0.2in}
\label{tab:datasets}
\end{table}

\subsection{Baselines}
In this paper, we compare our proposed GNN-based method to two other commonly used graph-based representation learning techniques. For both of the baseline techniques, the \gls{ssgnn} graph construction method is used to generate their input.

\textbf{\gls{dnn}} is a commonly used method for learning embeddings.

\textbf{\gls{gcn}} is a specific kind of Convolution Neural Network (CNN)~\cite{schmidhuber2015deep} that behaves similarly to the GNN by including the message passing perspective in the learning equation. The main difference between GCN and GNN is in the hidden layers of these architectures. The GCN stacks several graph convolution layers to extract a high-level node vector. On the other hand, the GNN contains Multi-Layer Perceptron (MLP)~\cite{haykin2004comprehensive} for the hidden layer representation to extract the node feature vector.

\textbf{\gls{gat}}~\cite{velivckovic2017graph} model fine-tunes the neighborhood message using self-attention layers and generates the attention coefficient $\alpha_{ij}$, which acts as a weight that defines how $node_j$ is related to  $node_i$. %The attention coefficient effectively improves edge connections and generates more fine-tuned message passing embeddings, making GAT a state-of-the-art algorithm in the research and production industries.

\subsection{Performance Metrics}
Since all datasets in HPC performance analytics contain continuous target values, we evaluate the performance of regression tasks by comparing the predicted value to the actual runtime value. We use the \gls{mse} loss that calculates the average squares of the error between the predicted and the true labels. %, and its output is always positive.
We evaluate our proposed pipeline's efficacy using three different HPC performance datasets where the main task is to \textit{predict the runtime}. 

Using different \gls{dnn} and graph-based models, we generate coarse-grained embeddings and evaluate their effectiveness by assessing how well a simple linear regression model performs when fed with the embeddings. The linear regression model achieves the target prediction by finding a linear relationship between the input and the output. The model adjusts the weights during the training phase to decrease the loss of the learning function and get better predictions. This model is frequently used in regression tasks such as predicting the weather or time series analysis because it is fast, efficient, and has less complex architecture than other models. Since this experiment aims to attribute any benefit to having superior embeddings, %assess the benefit of our proposed embedding learning technique, 
we keep the prediction task's model simple. % so that we can attribute any benefit to having superior embeddings.%We used the implementation of the linear regression model by sklearn.

\subsection{Hyper-Parameter Tuning}
\begin{table}[t]
\footnotesize
\caption{Hyper-parameters for different models.}
\label{table:Hyperparameters}
\renewcommand{\arraystretch}{1.2}
\centering
\begin{tabular}{|l|p{3cm}|p{2cm}|}
\hline
% \rowcolor{grey!20}
Model & Hyper-parameters & Search range \\ \hline
\multirow{2}{*}{DNN and Graph-Based} 
    &Hidden Layer Dimension &[25, 600]\\\cline{2-3}
    &Learning Rate	& [1e^{-5}, 1e^{-1}]\\ \cline{2-3}
&Dropout	&[0,1]\\ \cline{2-3}
&Optimizers	 &[Adam, Adagrad, Adadelta, SGD, RMSprop]\\ \cline{2-3}
&Activation function	 &[relu, elu,  leaky\_relu]\\ \hline

\multirow{2}{*}{Graph-Based} 

   & Hidden Layer Aggregation	&[pool,mean,gcn]\\ \cline{2-3}
&Self-Supervision Conv. Layer activation function&[relu, elu, leaky\_relu, sigmoid, tanh]\\ \cline{2-3}
&Number of Attention Heads
(GAT model only)	&[1,2]\\ \hline
\end{tabular}
  \vspace{-0.2in}
\end{table}
To achieve the best hyper-parameters, we take advantage of the Optuna framework~\cite{akiba2019optuna}. Optuna is a widely used hyper-parameter optimization framework that automatically and efficiently searches for the best parameters using state-of-the-art algorithms. Optuna also handles large search spaces through parallelization, enables distributed training across multiple CPUs and GPUs, and creates a trial history that can be visualized easily.
The \gls{dnn} and graph-based model parameters are optimized using Optuna in all experiments. Specifically, the model parameters to tune for the \gls{dnn} model are the number of hidden neurons, convolution layers, dropout rate, and learning rate. On the other hand, the Graph-Based models have extra parameters such as node aggregation and attention layers. Table~\ref{table:Hyperparameters} summarizes the hyperparameters for all the evaluated models in this paper.

% \begin{table}[t]
% \footnotesize
% \renewcommand{\arraystretch}{1.2}
% \centering
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% &Dataset	&Samples	&Features	&Domain	&Target	&Evaluation \\ \hline

% \end{tabular}
% \caption{Hyper-parameters search summary.}
% \label{table:Hyperparameters}
% \vspace{-0.2in}
% \end{table}
\subsection{Cross-Validation}
Researchers frequently use the cross-validation technique to estimate the model generalization over the whole dataset by randomly splitting the train/test sets multiple times and evaluating the model by averaging the results. In all experiments, we use K-fold, where K is equal to five, dividing the data into five train/test splits, generating five different results. Those five splits are randomly chosen to cover the entire dataset without changing anything in the actual data. Then we calculate the mean and standard deviation to get the generalized model performance and range. We ensure that the train and the test sets are disjoint.
 
 \subsection{Model and Embedding Assessment }
We assess the model from multiple perspectives to validate our approach. First, to validate the model’s ability to learn, we train the model to predict the value, look out for the training loss, and compare it to the testing loss to check if the model can learn and do feature extraction on the input. Then we consider the difference between training and testing losses and see the model’s ability to generalize. If the model is overfitting, we apply drop-out layers and L2 regularization.
Second, we use the same approach as the first step after making sure the model can learn. Still, instead of noticing the model performance, we extract the model embeddings through the hidden layer before the final prediction layer. Then we use those embeddings on a simpler model such as linear regression to calculate the change in performance and assess how effective the generated embeddings are.


==> results.tex <==
\subsection{Impact of Graph Representation}
\begin{table}[t]
\footnotesize
\caption{The results for the datasets, we used MSE loss and Percentage improvement as the evaluation metrics.}
\renewcommand{\arraystretch}{1.2}
\centering
\begin{tabular}{|p{2.3cm}|c|p{0.85cm}|p{1cm}|}
\hline
% \rowcolor{grey!20}
Dataset	&Catalyst	&Vulcan	&Cab		\\ \hline
DNN	&21.69	&617.64	&140.96		\\ \hline
GCN-MP	&22.28	&510.12	&142.16		\\ \hline
GAT	&39.07	&536.05	&133.85		\\ \hline
SSGNN	&16.39	&\textbf{455.69}	&131.52		\\
Improvement	&24.4\%	&26.34\%	&6.6\%	\\
\hline

SSBGNN	&\textbf{10.46}	&477.49	&\textbf{122.73}	\\ 
Improvement	&51.77\%	&22.8\%	&12.93\%	\\\hline
\end{tabular}
\vspace{0.05in}
\label{table:Datasets Eval}
% \vspace{-1in}
  \vspace{-0.2in}
\end{table}
The objective of this experiment is to test our initial hypothesis that using a graph structure to describe a performance dataset improves a predictive regression model's effectiveness. In this experiment, we compare five different models for three different applications, and Table~\ref{table:Datasets Eval} summarizes their performance using their respective best hyper-parameters. From Table~\ref{table:Datasets Eval}, we can observe that, on average, the graph-based representation learning approach outperforms DNN (baseline). This result can be explained by the fact that the graph-based models leverage explicit relationships between samples and features expressed in a graph structure, thus performing better than a regular DNN. DNN models can implicitly leverage higher-order correlations through connections across multiple layers; however, our experiments demonstrate that explicitly modeling the relations between data samples in \gls{ping} improves the effectiveness of a predictive regression model.

\subsection{Impact of Missing Data}
\begin{figure}[t]
\centering
  \includegraphics[width=\columnwidth]{figs/HPC-Models-Eval-.png}
\caption{Summary of evaluation of the five models on the HPC datasets: the y-axis represents the Normalized RMSE value. The X-axis presents the dataset names and the percentage of missing values per dataset.
}
  \label{fig:HPC-Eval}
  \vspace{-0.2in}
\end{figure}
The objective of this experiment is to evaluate the impact of the \gls{ping} formulation on the performance of regression tasks when missing data is present. The rationale for conducting this experiment is that streaming \gls{hpc} performance monitoring systems often miss recording feature values or cannot measure target values (unlabeled) until the application ends. To study the impact of missing data on the effectiveness of graph-based representation learning techniques, we randomly inject missing values (NaN) in 5\%, 10\%, 15\%, 20\%, and 25\% of the samples and compare the generated embeddings from DNN, \gls{ssgnn}, \gls{ssbgnn}, GCN-MP, and GAT. The GCN-MP and GAT methods use the graph constructed using our proposed \gls{sgc} method.

From Figure~\ref{fig:HPC-Eval}, we can observe that: (1) Our proposed approaches, \gls{ssgnn} and \gls{ssbgnn}, improve the prediction performance compared to all other models across all datasets in 16 out of the 18 experiments.
(2) The graph-based representation learning approaches outperform DNN, which reveals the proposed representation learning method's effectiveness and confirms the usefulness of the relations between data samples. 
(3) Our proposed automated edge-inference-based GNN method outperforms GCN's sum-based convolutional message passing across neighbors and GAT's attention-based aggregation strategy in 16 out of the 18 experiments, proving GNN to be a better method for capturing the complex relationships among the samples than GCN or GAT in the context of \gls{hpc}.

\noindent
% \textbf{Online Prediction:} Another significant benefit of graph representation is online prediction. New samples fed to the model in an online manner first sees the similar samples in previous data that the model has trained on. Then creates edges between the existing nodes and the new sample to build the graph and get enhanced predictions since the model leverages their relationship.
\subsection{Abalation Study}

\textbf{\textcolor{red}{Minimum Number of neighbours, $N$}}

In both of the SGC and BGC approach, we introduce an user defined property minimum number of neighbours, which defines the minimum numbers of N neighbours of a node in the graph. This property maintains the connectivity of the graph and removes the potential risk of generating a disconnected graph . A sample's closest distance when computing cosine distance is the sample itself. Thus we have self loops for all of the nodes of that generated graph. So, we take the top $N + 1$ neighbours instead of the $N$. Before generating the graph, we remove those self loops from the graph as mentioned both in \ref{alg:scg} \& \ref{alg:bgc}

\textbf{\textcolor{red}{Choosing SCG over BGC}}

Our study finds that, despite of efficient memory improvements in \textbf{BGC} than that of \textbf{SCG}, \textbf{BGC} isn't suitable for very small datasets. The reason behind that, there is a potential risk of generating single node graphs in some clusters due to scarcity of samples in the clusters. Our study shows that more than 600 samples in a dataset is a safe number of samples to conduct BGC approach of that dataset.  

\subsection{Computational Overhead}
We evaluate the computational overhead to ensure the feasibility of the graph representation learning method and its usage in the production environment. Figure \ref{fig:TrainingTime} reports the average of multiple training runs for 500 epochs. The overhead for graph-based methods include that of the initial \gls{ping} construction. 
\begin{figure}[t]
\centering
  \includegraphics[width=\columnwidth]{figs/TrainingTime.pdf}
\caption{Training time for each model based on 500 epoch, the Y-axis represents the model name, and the X-axis represents time in seconds.
}
  \label{fig:TrainingTime}
  \vspace{-0.2in}
  \end{figure}

From Figure~\ref{fig:TrainingTime}, we can observe that as the graph-based methods include an extra step of constructing the initial graph, on average, they take longer to train. Since this additional step brings significant performance improvement presented in Figure~\ref{fig:HPC-Eval}, this can be a worthy trade-off. Compared to this automated solution, others use manual feature engineering that needs a human to provide fine-tuned input. We also observe that \gls{ssbgnn} takes significantly longer than other models because it works on batches of graphs constructed using the \gls{bgc} method. Consequently, the sequential implementation of the graph batch loader API in DGL becomes a bottleneck for the training phase. However, since \gls{ssbgnn} uses batch training, we can accelerate the training time by distributing the training process across multiple GPUs, dramatically decreasing the training time. We leave this optimization for future. % work.

\subsection{Discussion }
Based on our evaluations, we can observe that our single-graph construction approach, \gls{ssgnn}, performs better for small datasets. On the other hand, the batched-graph construction approach \gls{ssbgnn} can achieve better performance since it clusters data together, thus making smaller, more memory-efficient graphs. If there are many patterns within the data, then the \gls{ssbgnn} produces fine-tuned graphs that can increase the model's performance.
Also, we observe that in the Cab dataset, the improvement percentage is low because the feature values do not vary significantly. Yet, the graph-based models achieve the best performance since our approach organizes similar data in a meaningful way, thus producing better embeddings.
Another significant benefit of graph representation is real-time prediction. Since the model has seen similar samples during training, it can connect new samples fed to the model in real-time with edges to the existing nodes and continue to augment the graph, thus enhancing the model's predictions. % since the model leverages their relationship.

